KISS: instrument description and performance

Kinetic inductance detectors (KIDs) have been proven as reliable systems for astrophysical observations, especially in the millimetre range. Their compact size enables to optimally fill the focal plane, thus boosting sensitivity. The KISS (KIDs Interferometric Spectral Surveyor) instrument is a millimetre camera that consists of two KID arrays of 316 pixels each coupled to a Martin-Puplett interferometer (MPI). The addition of the MPI grants the KIDs camera the ability to provide spectral information in the 100 and 300 GHz range. In this paper we report the main properties of the KISS instrument and its observations. We also describe the calibration and data analysis procedures used. We present a complete model of the observed data including the sky signal and several identified systematics. We have developed a full photometric and spectroscopic data analysis pipeline that translates our observations into science-ready products. We show examples of the results of this pipeline on selected sources: Moon, Jupiter and Venus. We note the presence of a deficit of response with respect to expectations and laboratory measurements. The detectors noise level is consistent with values obtained during laboratory measurements, pointing to a sub-optimal coupling between the instrument and the telescope as the most probable origin for the problem. This deficit is large enough as to prevent the detection of galaxy clusters, which were KISS main scientific objective. Nevertheless, we have demonstrated the feasibility of this kind of instrument, in the prospect for other KID interferometers (such as the CONCERTO instrument). As this regard, we have developed key instrumental technologies such as optical conception, readout electronics and raw calibration procedures, as well as, adapted data analysis procedures.

==> authors.tex <==
\author{
    J.~F. Mac\'ias-P\'erez\inst{\ref{LPSC}}\thanks{Corresponding author: J. F. Mac\'ias-P\'erez, \url{macias@lpsc.in2p3.fr} \& M. Fern\'{a}ndez-Torreiro, \url{mfernandez@lpsc.in2p3.fr} } 
    \and M. Fern\'{a}ndez-Torreiro\inst{\ref{LPSC}, \ref{IAC}, \ref{ULL}}\href{https://orcid.org/0000-0002-6805-9100}{\textcolor{orcidlogocol}{\aiOrcid}}
    \and A. Catalano\inst{\ref{LPSC}}
    \and A. Fasano \inst{\ref{Neel}, \ref{IAC}, \ref{ULL}} 
	\and M. Aguiar \inst{\ref{IAC}, \ref{ULL}}
	\and A. Beelen\inst{\ref{LAM}} 
	\and A. Benoit \inst{\ref{Neel}} 
	\and A. Bideaud \inst{\ref{Neel}}
    \and J. Bounmy \inst{\ref{LPSC}}
	\and O. Bourrion \inst{\ref{LPSC}}
	\and M. Calvo \inst{\ref{Neel}}
    \and J.~A. Castro-Almaz\'an \inst{\ref{IAC}, \ref{ULL}}
	\and P. de Bernardis\inst{\ref{Roma}} 
	\and M. De Petris\inst{\ref{Roma}}
    %\and F. D\'esert\inst{\ref{IPAG}}
	\and A. P. de Taoro \inst{\ref{IAC}, \ref{ULL}}
	\and G. Garde \inst{\ref{Neel}}
    \and R.~T. G\'{e}nova-Santos \inst{\ref{IAC}, \ref{ULL}}
	\and A. Gomez\inst{\ref{CAB}}
	\and M. F. G\'{o}mez-Renasco \inst{\ref{IAC}, \ref{ULL}} 
	\and J. Goupy \inst{\ref{Neel}} 
	\and C. Hoarau\inst{\ref{LPSC}}
	\and R. Hoyland \inst{\ref{IAC}, \ref{ULL}} 
	\and G. Lagache\inst{\ref{LAM}} 
	\and J. Marpaud\inst{\ref{LPSC}} 
	\and M. Marton\inst{\ref{LPSC}} 
    \and S. Masi\inst{\ref{Roma}} 
	\and A. Monfardini \inst{\ref{Neel}}
    \and M.~W. Peel \inst{\ref{Imperial}, \ref{IAC}, \ref{ULL} }
	\and G. Pisano \inst{\ref{Cardiff}}  
	\and N. Ponthieu\inst{\ref{IPAG}} 
	\and R. Rebolo \inst{\ref{IAC}, \ref{ULL}, \ref{CSIC}} 
    \and S. Roni\inst{\ref{LPSC}}
	\and S. Roudier\inst{\ref{LPSC}}
	\and J.~A. Rubi\~no-Mart\'in\inst{\ref{IAC}, \ref{ULL}}
	\and D. Tourres\inst{\ref{LPSC}} 
	\and C. Tucker \inst{\ref{Cardiff}}
    \and T. Viera-Curvelo \inst{\ref{IAC}, \ref{ULL}}
    \and C. Vescovi \inst{\ref{LPSC}}
}

\institute{
	Laboratoire de Physique Subatomique et de Cosmologie, Universit\'e Grenoble Alpes, CNRS/IN2P3, 53, avenue des Martyrs, Grenoble, France
	\label{LPSC}
    \and
	Instituto de Astrofísica de Canarias, C/Vía Láctea s/n, E-38205 La Laguna, Tenerife, Spain
	\label{IAC}
    \and
    Departamento de Astrof\'{\i}sica, Universidad de La Laguna, 
    E-38206 La Laguna, Tenerife, Spain
    \label{ULL}
	\and
	Institut N\'eel, CNRS and Universit\'e Grenoble Alpes, France
	\label{Neel}
    \and
	Aix Marseille Universit\'e, CNRS, LAM (Laboratoire d'Astrophysique de Marseille) UMR 7326, 13388, Marseille, France
	\label{LAM}
	\and
	Dipartimento di Fisica, Sapienza Universit\`a di Roma, Piazzale Aldo Moro 5, I-00185 Roma, Italy
	\label{Roma}
    \and
    Centro de Astrobiolog\'{\i}a (CSIC-INTA), Torrejón de Ardoz, 28850 Madrid, Spain
    \label{CAB}
	\and
    Imperial College London, Blackett Lab, Prince Consort Road, London SW7 2AZ, UK
    \label{Imperial}
    \and
	Astronomy Instrumentation Group, University of Cardiff, UK
	\label{Cardiff}
    \and
	Univ. Grenoble Alpes, CNRS, IPAG, F-38000 Grenoble, France 
	\label{IPAG}
    \and
    Consejo Superior de Investigaciones Cient\'{\i}ficas, E-28006 Madrid, Spain
    \label{CSIC}
}	
